On Defeating Graph Analysis of Anonymous Transactions

In a ring-signature-based anonymous cryptocurrency, signers of a transaction are hidden among a set of potential signers, called a ring, whose size is much smaller than the number of all users. The ring-membership relations specified by the sets of transactions thus induce bipartite transaction graphs, whose distribution is in turn induced by the ring sampler underlying the cryptocurrency. Since efficient graph analysis could be performed on transaction graphs to potentially deanonymise signers, it is crucial to understand the resistance of (the transaction graphs induced by) a ring sampler against graph analysis. Of particular interest is the class of partitioning ring samplers. Although previous works showed that they provide almost optimal local anonymity, their resistance against global, e.g. graph-based, attacks were unclear. In this work, we analyse transaction graphs induced by partitioning ring samplers. Specifically, we show (partly analytically and partly empirically) that, somewhat surprisingly, by setting the ring size to be at least logarithmic in the number of users, a graph-analysing adversary is no better than the one that performs random guessing in deanonymisation up to constant factor of 2.

==> 0-format_infos.tex <==
% !TEX root = main.tex

\begin{minipage}{\textwidth}
\ifnum\showcomments=1
You are using \ifnum\style=0 ARTICLE \fi\ifnum\style=1 LNCS \fi
\ifnum\style=2 ACM \fi\ifnum\style=3 USENIX\fi\ifnum\style=4 IEEE \fi
\ifnum\style=5 SCIENDO \fi style with
\ifnum\paperversion=0 ANONYMOUS \fi\ifnum\paperversion=1 CAMERAREADY \fi
\ifnum\paperversion=2 FULLVERSION \fi mode.


\noindent Textheight: \uselengthunit{in}\printlength{\textheight} / \uselengthunit{mm}\printlength{\textheight}\\
Linewidth: \uselengthunit{in}\printlength{\linewidth}/\uselengthunit{mm}\printlength{\linewidth}\\
\noindent Pageheight:\uselengthunit{in} \printlength{\pdfpageheight}/\uselengthunit{mm}\printlength{\pdfpageheight}\\
Pagewidth: \uselengthunit{in}\printlength{\pdfpagewidth}/\uselengthunit{mm}\printlength{\pdfpagewidth}




\uselengthunit{pt}
\noindent Baselineskip: \printlength{\baselineskip}\\
\makeatletter
Fontsize: \f@size pt
\makeatother




\noindent Font: \fontname\font
\end{minipage}

\clearpage


==> 0-paper_settings.tex <==
% !TEX root = main.tex

% General Settings

\setlength\emergencystretch{3em}

% --- -----------------------------------------------------------------
% --- AutoRef Settings.
% --- -----------------------------------------------------------------
\def\algorithmautorefname{Algorithm}
\def\appendixautorefname{Appendix}
\def\corollaryautorefname{Corollary}
\def\definitionautorefname{Definition}
\def\exampleautorefname{Example}
\def\lemmaautorefname{Lemma}
\def\linesautorefname{Line}
\def\propositionautorefname{Proposition}
\def\sectionautorefname{Section}
\def\subfigureautorefname{Figure}
\def\subsectionautorefname{Section}
\def\theoremautorefname{Theorem}

==> blank.tex <==
% !TEX root = main.tex

\section{Preliminaries}

Let $H = \tuple{V_H, E_H}, K = \tuple{V_K, E_K}$ be hypergraphs.
If $K$ is a subgraph of $H$, \ie, $V_K \subseteq V_H$ and $E_K \subseteq E_H$, we write $K \subseteq H$.
$H \setminus K$ denotes the graph obtained by removing all nodes contained in $K$ from $H$, \ie,
\begin{align*}
    H \setminus K := \tuple{V_H \setminus V_K, \set{E \setminus V_K}_{E \in E_H}}.
\end{align*}

\section{Problem Statement}


Let $k,n \in \NN$ such that $k \subseteq n$.
Let
\begin{align*}
    \mathcal{H}_{k,n} := \set{
        H = \tuple{V, E = \set{E_v}_{v \in V}}:
        |V| = n \land
        \forall v \in V, v \in E_v \subseteq_k V
    }
\end{align*}
be the set of $k$-regular hypergraphs with $n$ nodes and $n$ (hyper)edges, where there exists at least one way to label each edge  with a unique node.
Such graphs arise naturally in the context of ring sampling.
Let $\Pi$ be a $(1,k)$-ring sampler over the universe $[n]$.
For $i \in [n]$, let $E_i \gets \Pi(i)$ be the ring sampled by signer $i$.
Then $\tuple{[n],\set{E_i}_{i \in [n]}} \in \mathcal{H}_{k,n}$.

Let $H \in \mathcal{H}_{k,n}$. We write $K < H$ if there exists $s < n$ such that $K \in \mathcal{H}_{k,s}$ and $K \subseteq H$.

We are interested in the following problems:
\begin{enumerate}
    \item Compute
    \[\Pr[H \sample \mathcal{H}_{k,n}]{\exists K < H}.\]
    Note that if there exists $K < H$,
    it means that the set of rings $E_K$ were created by the signers in $V_K$.
    In other words, the rings in $E_H \setminus E_K$ were created by the signers in $V_H \setminus V_K$.
    An (unbounded) adversary can deanonymize the signers (reducing the size of their anonymity sets) by ``partitioning'' $H$ into $K$ and $H \setminus K$. We conjecture that the above probability is upper-bounded by $O(2^{-k})$.

    \item Let $H \in \mathcal{H}_{k,n}$ such that there exists $K < H$. What is the complexity of finding one such $K$? This question is interesting as it is where computational hardness might start to kick in. So far we were always considering anonymity information-theoretically. If this problem turns out to be computationally hard, then even if the information-theoretic anonymity turns out to be low (\ie, the probability in Problem 1 is high), the computational anonymity might be still high. We conjecture that the problem cannot be solved in time $o(2^k) \cdot
    \poly[n]$.
\end{enumerate}

\section{Case $k=2$}

In the case $k=2$, $k$-regular hypergraphs degenerate into ordinary graphs, and $\mathcal{H}_{2,n}$ is simply the set of graphs with $n$ nodes and $n$ edges where the $i$-th node belongs to the $i$-th edge. A classical textbook result states that any $H \in \mathcal{H}_{2,n}$ must contain a cycle. Therefore, unless $H$ is an $n$-cycle, there must exist $K < H$. We therefore have
\begin{align*}
    &\Pr[H \sample \mathcal{H}_{k,n}]{\exists K \in \mathcal{H}_{k,s} \suchthat s < n \land K \subseteq H} \\
    = &1 - \Pr{\text{$H$ is an $n$-cycle}} \\
    = &1 - \frac{(n-1)!}{(n-1)^n} \\
    \geq &1 - \frac{(n-1)^{n}}{e^{n-2} (n-1)^n} \\
    = &1 - e^{2-n} \\
    \to &1~\text{as $n \to \infty$}.
\end{align*}

Furthermore, there exists an $O(n^2)$-time algorithm $\mathsf{SubgraphFinding}$ which solves Problem 2.
Let $H = \tuple{V = \set{v_i}_{i=1}^n, E = \set{E_v}_{v \in V}}$.
Since $v \in E_v$ for all $v \in V$, without loss of generality, let $E_v = (v, u_v)$ for some $u_v \in V$.
The algorithm $\mathsf{SubgraphFinding}$ does the following:

\begin{figure*}[h]
    \centering
    \procedure[space=auto]{$\mathsf{SubgraphFinding}(H)$}
    {
        \pcforeach v \in V \pcdo \\
        w := v \\
        V' := \set{w} \\
        \pcwhile u_w \notin V' \pcdo \\
        V' := V' \cup \set{u_w} \\
        E' :=  E' \cup \set{(w, u_w)} \\
        w := u_w \\
        \pcendwhile \\
        E' :=  E' \cup \set{(w, u_w)} \\
        \pcif |V'| < n \pcthen \\
        \pcreturn (V', E') \\
        \pcendif \\
        \pcendfor \\
        \pcreturn \bot
    }
\end{figure*}

Observe that just before the if-condition we have $|V'| = |E'| \subseteq n$.
Due to the existence of $K < H$, there must exist a cycle of length $s < n$.
Therefore the if-condition must be satisfied for some $v$ in the for-loop, and the algorithm outputs a desired subgraph.
As the algorithm makes at most $n$ traversals, each through at most $n$ nodes, the running time is upper-bounded by $O(n^2)$.

\section{Random Ideas}

\begin{conjecture}
    Let $H \in \mathcal{H}_{k,n}$. If $K_0, K_1 < H$, then $K_0 \cap K_1, K_0 \setminus K_1, K_1 \setminus K_0 < K_b$ for $b \in \bits$.
\end{conjecture}


==> fig_outline.tex <==
% !TEX root = main.tex

\begin{figure*}[t]
\newcommand{\botleq}{\begin{sideways}\ensuremath{\leq}\end{sideways}}
\newcommand{\boteq}{\begin{sideways}\ensuremath{=}\end{sideways}}
\centering
\fbox{
\begin{tikzpicture}
\node (reg-sc) at (0,5.2) {$\displaystyle \sum_{C \in P} \Pr[\vec{G} \gets \vec{\cG}^{\regtag}_{k,|C|}]{\vec{\rvG} \notin \SC}$};
\node[label=right:{\small Direct Inspection}] (1) at (0,4.5) {$\boteq$};
\node (reg-part) at (0,3.8) {$\displaystyle \sum_{C \in P} \Pr[G \gets \cG^{\RegSamp[P,k]}_{C,C}]{\ID{\rvG} \notin \SC}$};
%\node (reg-part) at (0,3.8) {$\displaystyle\sum_{C \in P} \Pr[G \gets \cG^{\RegSamp[P,k]}_{C,C}]{G \neq \core{G}}$};
\node[label=right:{\small\cref{thm:core}}] (1) at (0,3.1) {$\botleq$};
\node (reg-bal) at (0,2.4) {$\displaystyle\Pr[G \gets \cG^{\RegSamp[P,k]}]{G \neq \core{G}}$};
\node[label=right:{\small\cref{thm:balance_is_upper_bound}}] (1) at (0,1.7) {$\botleq$};
\node (reg) at (0,1) {$\displaystyle\Pr[G \gets \cG^{\RegSamp[P,k]}_{U,M}]{G \neq \core{G}}$};

\node (bin-sc) at (6,5.2) {$\displaystyle \sum_{C \in P} \Pr[\vec{G} \gets \vec{\cG}^{\bintag}_{p,|C|}]{\vec{\rvG} \notin \SC}$};
\node[label=right:{\small Direct Inspection}] (1) at (6,4.5) {$\boteq$};
\node (bin-part) at (6,3.8) {$\displaystyle \sum_{C \in P} \Pr[G \gets \cG^{\BinSamp[P,p]}_{C,C}]{\ID{\rvG} \notin \SC}$};
\node[label=right:{\small\cref{thm:core}}] (1) at (6,3.1) {$\botleq$};
\node (bin-bal) at (6,2.4) {$\displaystyle\Pr[G \gets \cG^{\BinSamp[P,p]}]{G \neq \core{G}}$};
\node[label=right:{\small\cref{thm:balance_is_upper_bound}}] (1) at (6,1.7) {$\botleq$};
\node (bin) at (6,1) {$\displaystyle\Pr[G \gets \cG^{\BinSamp[P,p]}_{U,M}]{G \neq \core{G}}$};

% \node[label=above:{\small\cref{conj:reg_leq_bin}}] (conj1) at (3,5.2) {$\leq$};
\node[label=above:{\parbox{7em}{\centering\small\cref{conj:reg_leq_bin},\\$p=p(C)=\frac{k}{|C|-1}$}}] (conj1) at (3,5.2) {$\leq$};
% \node[label=above:{\small\cref{conj:bin_upper_bound}}] (conj2) at (9,5.2) {$\leq$};
\node[label=above:{\parbox{7em}{\centering\small\cref{conj:bin_upper_bound},\\$|C| \leq n$ for $C \in P$}}] (conj2) at (9,5.2) {$\leq$};
\node (bound) at (12,5.2) {$\displaystyle |P| \tuple{1 - e^{-2e^{\ln n - k}}}$};
\end{tikzpicture}}
\caption{Overview of our results.}
\label{fig:outline}
\end{figure*}


==> new_part.tex <==
% !TEX root = main.tex

\section{Partitioning Sampler with Replacement}

The partitioning sampler described in~\cite{PoPETs:RELSY21} samples a fixed number of decoys for each signer from the respective chunk, which makes the analysis of its induced transaction graphs tedious. In the following, we define an analogue of the partitioning sampler where, for each signer, each member in the respective chunk is to be chosen as decoy with a fixed probability.


We focus on the simple case where there is only one public partition of $U$. The general case with a distribution of partitions can be handled with generic techniques~\cite{PoPETs:RELSY21}. Let $P$ be a partition of $U$ and $\chi \in [0,1]$ be a probability. Our NEW partitioning sampler $\Pi_{P, \chi}$ is defined as follows.

\begin{quote}
    $\Pi_{P, \chi}(S)$:
    Initiate $R := S$.
    For each $s \in S$, let $C_s \in P$ be the unique chunk containing $s$.
    For each $s \in S$ and each $d \in C_s\setminus s$, run $R := R \cup \set{d}$ with probability $\chi$.
    Output $R$.
\end{quote}

In case $\sdv$ is a single-signer distribution, letting $\chi=\frac{k-1}{|C_s|-1}$ for some $k\geq 1$, our new sampler is analogous to the $(1,k)$-partitioning sampler in \cite{PoPETs:RELSY21}, where the expected ring size is fixed at $k$, and the actual ring size is allowed to vary under $Bin(|C_s|-1,\chi) + 1$.

\begin{theorem}
    Let $n, m \in \NN$ with $n \leq m$,
    $\sdv$ be a single-signer distribution,
    $P$ be a partition of $U$ such that $|C| \geq m$ for all $C \in P$, and
    $\chi \geq n/m$.
    Suppose that for all $C \in P$, all $s \in C$, it holds that $\abs{\Pr{\rv S = \set{s}} - \mu_C} \leq \epsilon_C$ for some $\epsilon_C \geq 0$.
    Let $\epsilon_P := \sum_{C \in P} |C| \epsilon_C$.
    Then
    \[
		\alpha[\sdv,\Pi_{P,\chi}] \geq \log n - \lg(\epsilon_P + 1).
    \]
\end{theorem}

\begin{proof}
	As the chunk containing $s$ is unique, we know that $\bigcup_{C \in P} (2^C \setminus \set{\emptyset})$ is the collection of all possible rings.
	Since the ring given by the sampler must contain the signer $s$, we have for all $R \in \bigcup_{C \in P} (2^C \setminus \set{\emptyset})$, 
	\begin{equation*}
		\Pr{\rv R = R \wedge s \notin R | \rv S = \set{s}} = 0.
	\end{equation*}
	If $s \in C \in P$, then each element in $C \setminus \set{s}$ has a probability $\chi$ to be included in $R \setminus \set{s}$.
	On the other hand, if $s \notin C \in P$, then we must have $R \notin 2^C \setminus \set{\emptyset}$.
	Therefore, for any $C \in P$, we have
	\begin{align*}
		&\Pr{\rv R = R \wedge s \in R | \rv S = \set{s}} \\
		=& \begin{cases}
			\chi^{|R|-1} (1-\chi)^{(|C|-1) - (|R|-1)} = \chi^{|R|-1} (1-\chi)^{|C|-|R|} & s \in C\\
			0 & s \notin C.
		\end{cases}
	\end{align*}
	Now, we analyze the anonymity of the sampler.
	\begin{align*}
		&2^{-\alpha[\sdv,\Pi_{P,\chi}]}
		= 2^{H_\infty(\sdv|\Pi_{P,\chi}(\sdv))} \\
		= &\sum_{R \in \bigcup_{C \in P} (2^C \setminus \set{\emptyset})} \max_{s} \Pr{\rv R = R | \rv S = \set{s}}\Pr{\rv S = \set{s}} \\
		= &\sum_{C \in P} \sum_{R \in (2^C \setminus \set{\emptyset})} \max_{s} (\Pr{\rv R = R \wedge s \in R | \rv S = \set{s}} + \Pr{\rv R = R \wedge s \notin R | \rv S = \set{s}}) \Pr{\rv S = \set{s}} \\
		\leq &\sum_{C \in P} \sum_{R \in (2^C \setminus \set{\emptyset})} \chi^{|R|-1} (1-\chi)^{|C|-|R|} \max_{s} \Pr{\rv S = \set{s}} \\
		= &\sum_{C \in P} \frac{1}{\chi} \left( \sum_{R \in 2^C} \chi^{|R|} (1-\chi)^{|C|-|R|} - \chi^{|\emptyset|} (1-\chi)^{|C|-|\emptyset|} \right) \max_{s} \Pr{\rv S = \set{s}} \\
		= &\sum_{C \in P} \frac{1}{\chi} \left( 1 - (1-\chi)^{|C|} \right) \max_{s} \Pr{\rv S = \set{s}} \\
		\leq &\sum_{C \in P} \frac{1 - (1-\chi)^{|C|}}{\chi} (\mu_C + \epsilon_C) \\
		\leq &\frac{m}{n} \sum_{C \in P} (\mu_C + \epsilon_C) \\
		= &\frac{m}{n} \sum_{C \in P} \frac{|C|}{|C|} (\mu_C + \epsilon_C) \\
		\leq &\frac{m}{n} \sum_{C \in P} \frac{|C|}{m} (\mu_C + \epsilon_C) \\
		= &\sum_{C \in P} \frac{|C|}{n} (\mu_C + \epsilon_C)\\
		= &\frac{\epsilon_P + 1}{n}. %\qedhere
	\end{align*}
\end{proof}



==> problem.tex <==
%!TEX root=main.tex
\section{Problem statement with bipartite graphs}
\begin{definition}
  Let $G=(V=(V_A,V_T),E)$ be an undirected bipartite graph, \ie $e_{i,j}=e_{j,i}$. We call $G$ a \emph{proper transaction graph} if the following holds:
  \begin{itemize}
    \item $\forall e_{i,j}\in E\,:\,(i\in V_A\vee j \in V_A)\wedge(i\in V_T \vee j \in V_T)$
    \item $\forall j \in V_T\,:\, \exists_n\ e_{i,j}\in E~s.t.~ i \in V_A$
    \item $|E|=n\cdot|V_T|$ (should be redundant)
  \end{itemize}
\end{definition}

\begin{definition}
  Let $G(V=(V_A,V_T),E)$ be a graph as before. W.l.o.g. we name an edge $e_{i,j}$ always as edge from $i\in V_A$ to $j\in V_T$. We say a subgraph $H=(W=(W_A,W_T)\subseteq V,F\subseteq E)$ is \emph{closed} if
  \begin{itemize}
    \item $|W_A|=|W_T|\geq n$
    \item $\forall j \in W_T\,:\, i\in W_A\ \forall\ e_{i,j}\in E$
  \end{itemize}
\end{definition}

\paragraph{Questions}
\begin{enumerate}
  \item What is the probability that $k$ users chose all their decoys amongst each other?
  \item What is the probability that a random proper transaction graph contains a closed subgraph of size $k$?
  \item What is the probability for two closed subgraphs $H$, $H'$ such that $H\subset H'$, $|H'|=k'$, $|H|=k$ and $k'-k<n$
\end{enumerate}


==> subgraphExistence.tex <==
%!TEX root=main.tex
\section{Problem statement with bipartite graphs}
\begin{definition}
  Let $G=(V=(V_A,V_T),E)$ be an undirected bipartite graph, \ie $e_{i,j}=e_{j,i}$. We call $G$ a \emph{proper transaction graph} if the following holds:
  \begin{itemize}
    \item $\forall e_{i,j}\in E\,:\,(i\in V_A\vee j \in V_A)\wedge(i\in V_T \vee j \in V_T)$
    \item $\forall j \in V_T\,:\, \exists_n\ e_{i,j}\in E~s.t.~ i \in V_A$
    \item $|E|=n\cdot|V_T|$ (should be redundant)
  \end{itemize}
\end{definition}

\begin{definition}
  Let $G(V=(V_A,V_T),E)$ be a graph as before. W.l.o.g. we name an edge $e_{i,j}$ always as edge from $i\in V_A$ to $j\in V_T$. We say a subgraph $H=(W=(W_A,W_T)\subseteq V,F\subseteq E)$ is \emph{closed} if
  \begin{itemize}
    \item $|W_A|=|W_T|\geq n$
    \item $\forall j \in W_T\,:\, i\in W_A\ \forall\ e_{i,j}\in E$
  \end{itemize}
\end{definition}

\noindent Two possibilities:
\begin{enumerate}
  \item[$X$] What is the probability that $k$ users chose all their decoys amongst each other?
  \item[$Y$] What is the probability that a random proper transaction graph contains a closed subgraph of size $k$?
\end{enumerate}

\section{Probability of spenders choosing within decoys within themselves}

We see the graph of transactions as a bipartite graph with the vertices on one side representing the transactions (and thus having exactly $n$ edges for simplification) and on the other side representing each possible spender in the system.
We describe the graph in a adjacency matrix of size $(l\times a)$, \ie rows describe transactions (and contain therefore exactly $n$  1s) and columns are spenders.
We define a subgraph $G=(V_s,V_{tx},E)$ as spanned by some transaction vertices, \ie a subgraph contains some transaction vertices, all edges to this vertices as well as all vertices connected with the transactions.
$V_{tx}$ contains all vertices representing transactions, $V_s$ all vertices representing accounts. We identify each vertex with its index in the adjacency matrix (either row or column).
W.l.o.g. we can assume that the matrix is ordered in a way such that the column number of a real spender matches the row number of the transaction it spends.
Further the transactions are sorted by \enquote{age} and we assume a fixed amount of transactions per block and a fixed amount of newly created accounts per block.

Let
\begin{description}
  \item[$l$] be the total number of transactions,
  \item[$a$] the number of accounts,
  \item[$n$] the ring size (fixed),
  \item[$g$] the size of the subgraph,
  \item[$I$] the set of row/column indices for the subgraph,
  \item[$b$] the number of transactions per block,
  \item[$d$] the number of newly created accounts per block and
  \item[$o$] the initial number of accounts in the system.
\end{description}

For a working system it is necessary that the initial number of accounts is at least $n$.
We denote by $I$ the set of column/row indices of the subgraph, \ie each element in $I$ denotes both a row and a column in the subgraph due to our previous sort of the matrix. Thus each index in the submatrix can be denoted by $(i_1,i_2)$ for $i_1,i_2\in I$. We further assume that $I$ is ordered.

Naturally, $g\leq n$ has to hold. This does not mean that actual spenders cannot be deanonymized entirely. This can happen when a closed subgraph of size $g$ contains another one of size $g-1$.

\begin{lemma}
  The number of accounts a spender at position $i$ can choose from is $d\cdot\lfloor\frac{i}{d}\rfloor + o$.
\end{lemma}

\begin{idea}
  Each block creates $d$ accounts and up to index $i$ there were $\lfloor \frac{i}{d}\rfloor$ blocks. Additionally there are $o$ initial accounts.
\end{idea}

\begin{lemma}
  Let $G=(V_s,V_{tx},E)$ be a subgraph as described above with $i\in V_s$ and $I$ denoting the indices in $V_s$.
  Let $X_{G,i}=1$ be the event that $i$ chooses all ring members within $V_s$. Let $j$ be the position of $i$ in $I$. The probability for $X=1$ is
  \begin{gather*}
    \Pr{X_{G,i}=1} = \binom{\min(g,m_{g,i}) }{n-1} \cdot \binom{d\cdot\lfloor \frac{i}{d}\rfloor + o -1}{n-1}^{-1},\\
    m_{g,i} = \begin{cases}
    (\max j\,|\,i_j \leq d\cdot\lfloor \frac{i}{d}\rfloor + o\wedge i_j \neq i) +1 & i > i_j \\
    \max j\,|\,i_j \leq d\cdot\lfloor \frac{i}{d}\rfloor + o\wedge i_j \neq i & else
    \end{cases}
  \end{gather*}
  when uniform sampling is used.
\end{lemma}

\begin{idea}
  The right binomial coefficient is just choosing the ring from all possibilities spender $i$ has.
  If $i$ can choose from enough accounts, it can choose from the whole subgraph and therefore has $g-1$ accounts to choose from. If this is not the case we use the number of available accounts within the subgraph that $i$ can choose from.
\end{idea}

Simplification

\begin{align*}
  & \binom{\min(g,m_{g,i})-1}{n-1} \cdot \binom{d\cdot\lfloor \frac{i}{d}\rfloor + o -1}{n-1}^{-1} =\\
  &  =
  \frac{[\min(g,m_{g,i})-1]! \cdot [d\cdot\lfloor \frac{i}{d}\rfloor + o -1 - n + 1]\cdot[n-1]!}{[\min(g,m_{g,i})-1 - n + 1]! \cdot [n-1
  ]![d\cdot\lfloor \frac{i}{d}\rfloor + o -1]!} \\
  &  =
  \frac{[\min(g,m_{g,i})-1]! \cdot [d\cdot\lfloor \frac{i}{d}\rfloor + o - n]}{[\min(g,m_{g,i}) - n ]! [d\cdot\lfloor \frac{i}{d}\rfloor + o -1]!} \\
  & = \prod_{k=1}^{n-1}\frac{\min(g,m_{g,i})-k}{d\cdot\lfloor \frac{i}{d}\rfloor + o -k}
\end{align*}

\begin{lemma}
  Let $G=(V_s,V_{tx},E)$ be a subgraph as described above with $I$ denoting the indices in $V_s$.
  Let $X=1$ be the event that all $X_{G,{i\in I}}=1$, \ie $G$ is a closed subgraph. Then the probability is
  \begin{align*}
    \Pr{X=1} = \prod_{i\in I}^{g-1} \Pr{X_{G,i}}
    % = \prod_{i=0}^{g-1} \prod_{k=1}^{n-1}\frac{\min(g,d\cdot\lfloor \frac{j+i}{d}\rfloor + o -j)-k}{d\cdot\lfloor \frac{j+i}{d}\rfloor + o -k}
  \end{align*}
  when uniform sampling is used.
\end{lemma}

Finding such a subgraphs equals finding $g$ accounts which are the actual spenders in $g$ transactions.

\begin{idea}
  We assume each spender samples independently from each other, \ie $X_{G,{i\in I}}$ are independent.
\end{idea}

A simpler version of the above results in using a partitioning sampler where the outer partition is done by \enquote{splitting} the universe of exisiting accounts by time into equally sized chunks (thereby ignoring the newest ones) and then sampling uniformly from these chunks.
This can be seen as a universe of fixed size, where each spender can choose every account in the universe, leading to

\begin{lemma}
  Let $G=(V_s,V_{tx},E)$ be a subgraph as described above
   with $i\in V_s$ and $I$ denoting the indices in $V_s$.
  Let $X_{G,i}=1$ be the event that $i$ chooses all ring members within $V_s$.
  \begin{align*}
    \Pr{X_g=1} &= \binom{g-1}{n-1}\cdot \binom{a-1}{n-1}^{-1} \\
    &= \prod_{j=1}^{n-1}\frac{g-j}{k-j}.
  \end{align*}
\end{lemma}

The probability for all accounts to choose within the \enquote{right} subgraph is thus
\begin{align*}
  g\cdot \prod_{j=1}^{n-1}\frac{g-j}{k-j}.
\end{align*}

% If a universe is spent completely, this obviously is a closed (sub)graph.
% Also a closed subgraph provides information if an account is actually already spent.
% On the other hand, it does not give information about in which transaction of the subgraph an account is spend.
% This can be done if we find two subgraphs of the desired property where the contained subgraph is at most $n-1$ smaller than the outer part.
%
% \begin{lemma}
%   Let $G=(V_s,V_{tx},E)$ be a closed subgraph in the universe of accounts. The probability that $G$ contains a subgraph itself of size $h$ is
% \end{lemma}

\begin{lemma}
  Let $V_s$ be a set of spenders. For any subset of size $g$ of this spenders, the probability that they form a closed subgraph when building transactions is \Pr{X_g=1}.
  Thus, the probability that any such closed subgraph can be upper-bounded by
  \begin{align*}\binom{|V_s|}{g}\cdot\Pr{X_g}&=\binom{|V_s|}{g}\cdot g\cdot
    \prod_{j=1}^{n-1}\frac{g-j}{a-j} \\
&= \frac{a!\cdot(a-n)!}{(a-g)!\cdot(g-n)!\cdot(a-1)!}\\
&=\frac{a\cdot(a-n)!}{(a-g)!\cdot(g-n)!}
  \end{align*}
\end{lemma}


==> subgraphs.tex <==
%!TEX root=main.tex
\section{Probabilietes for Closed Subgraphs}
We first consider a fixed universe size $\ell=|G|$, $G=((V_A,V_T),E)$ and a uniform sampling of decoys. This would match uniform sampling within a partition.

\begin{itemize}
  \item[$\ell$] universe size
  \item[$h$] size of subset $H\subseteq V_A$
\end{itemize}

\begin{lemma}Let $X_{H,i}$ be the event that for a spender $i\in H$, it chooses all decoys within $H$ and $X_H$ that all spenders in $H$ choose their decoys within $H$. Then it holds
  \begin{align*}
    \Pr{X_{H,i}=1} = \binom{h-1}{n-1}\binom{l-1}{n-1}^{-1}
  \end{align*}
  and
  \begin{align*}
    \Pr{X_H}=\Pr{\bigwedge_{i\in H} X_{H,i}=1}=\Pr{X_{H,i}}^l.
  \end{align*}
 This is the probability that all spenders in $H$ choose their decoys also in $H$.
\end{lemma}
This is simply the number of possible selections of $n-1$ decoys in $H$ divided by the number of possible selections of $n-1$ decoys in $G$.


\begin{lemma} Let $Y_h$ be the event that a proper transaction graph $G$ contains at least one closed subgraph of size $h$. Then
  \begin{align*}
    \Pr{Y_h}\leq \binom{l}{h}\Pr{X_H}
  \end{align*}
  for arbitrary $H$ with $H=h$.
\end{lemma}

\begin{idea}
  Given the precondition, \Pr{H} is the same for all $H$ of size $H$. Therefore, we can estimae \Pr{Y_h} by multiplying the probability that for a subset $H\subseteq V_A$, all spenders choose within $H$ with the number possibilities to choose $H$.
  It is an overestimation as there might be two closed subgraphs of size $h$ which are counted twice.
\end{idea}

\begin{lemma}
  Let $H'$ be a closed subgraph as before and $H\subset H'$ such that $h'-h<n$. Then
  \begin{align*}
    \Pr{X_H\wedge X_{H'}} =\left[\binom{h'-1}{n-1}\binom{l-1}{n-1}^{-1}\right]^{h'-h}\cdot\left[\binom{h-1}{n-1}\binom{l-1}{n-1}^{-1}\right]^{h}
  \end{align*}
\end{lemma}
\begin{idea}
  If an element in $H$ selects decoys in $H$ it also selects decoys in $H'$, so we can use the idea from before again.
\end{idea}

\begin{lemma}
  Let $Y_{h,h'}$ be the event that a proper transaction graph $G$ contains at least one closed subgraph of size $h'$ which itself contains a subgraph of size $h$. Then
  \begin{align*}
    \Pr{Y_{h,h'}} \leq \binom{l}{h'}\cdot\left[\binom{h'-1}{n-1}\binom{l-1}{n-1}^{-1}\right]^{h'-h}\cdot\binom{h'}{h}\cdot\left[\binom{h-1}{n-1}\binom{l-1}{n-1}^{-1}\right]^{h}
  \end{align*}
\end{lemma}

